The post-disk (or primordial) spin distribution of M dwarf stars

We investigate the influence of an accretion disk on the angular momentum (AM) evolution of young M dwarfs, which parameters govern the AM distribution after the disk phase, and whether this leads to a mass-independent distribution of SAM. We find that above an initial rate $\dot{M}_\mathrm{crit} \sim 10^{-8}~\mathrm{M_\odot/yr}$ accretion "erases" the initial SAM of M dwarfs during the disk lifetime, and stellar rotation converges to values of SAM that are largely independent of initial conditions. For stellar masses $> 0.3~\mathrm{M_\odot}$, we find that observed initial accretion rates $\dot{M}_\mathrm{init}$ are comparable to or exceed $\dot{M}_\mathrm{crit}$. Furthermore, stellar SAM after the disk phase scales with the stellar magnetic field strength as a power-law with an exponent of $-1.1$. For lower stellar masses, $\dot{M}_\mathrm{init}$ is predicted to be smaller than $\dot{M}_\mathrm{crit}$ and the initial conditions are imprinted in the stellar SAM after the disk phase. To explain the observed mass-independent distribution of SAM, the stellar magnetic field strength has to range between 20~G and 500~G (700~G and 1500~G) for a 0.1~$\mathrm{M_\odot}$ (0.6~$\mathrm{M_\odot}$) star. These values match observed large-scale magnetic field measurements of young M~dwarfs and the positive relation between stellar mass and magnetic field strength agrees with a theoretically-motivated scaling relation. The scaling law between stellar SAM, mass, and the magnetic field strength is consistent for young stars, where these parameters are constrained by observations. Due to the very limited number of available data, we advocate for efforts to obtain more such measurements. Our results provide new constraints on the relation between stellar mass and magnetic field strength and can be used as initial conditions for future stellar spin models, starting after the disk phase. (shortened)

==> REF_reply.tex <==
% The authors employ parametric models of the angular momentum (AM) evolution of young forming M dwarfs still magnetically interacting with their surrounding accretion disk to investigate their specific angular momentum (SAM) distribution at the end of the disk lifetime (< 10 Myr). Observations of the Upper Scorpius association, whose age is around 10 Myr and most accretion disks should have dissipated, that its SAM distribution does not strongly depend on stellar mass (Somers et al. 2017). The authors aim at understanding this behavior by running simulations of the AM evolution of young M dwarfs and investigate which factors could determine a mass-independent SAM distribution. Their AM evolution models are largely based on works such as Matt et al. (2010) and Gallet et al. (2019). They nevertheless introduce a novel aspect in their simulations by using an implicit disk evolution model that self-consistently computes the disk accretion rate, instead of assuming an accretion temporal evolution loosely based on observations as in the cited works. By running a statistically relevant number of simulations (around 500), they are able to: 1) determine under which conditions the final SAM of M dwarfs retains information about the initial angular momentum distribution at 1 Myr; 2) mainly ascribe the median and standard deviation of the observed mass-independent SAM distributions to the intensity of the stellar magnetic field, with higher stellar masses requiring stronger magnetic fields. They also show that the magnetic field range required by their models matches relatively well the range of observed large-scale dipolar field strengths.
% Since I am acting as a second referee for the submitted paper, my report is largely based on the last revised submitted version already containing the corrections made to answer to the first referee's comments.
% Thanks to the first referee’s suggestions, I think that there has been a noticeable improvement from the previous revisions to the last submitted version. The range of the free parameters of the AM evolution models is better constrained and observationally motivated. If I interpret correctly the results, the use of an initial mass accretion rate relation with the stellar mass (Eq. 5) based on observations of flat-spectrum sources transiting from Class I to Class II helped to limit the influence of the initial conditions of the models and to put stronger constraints on the magnetic field values, especially the stellar mass/magnetic field relation, which is one of the novel conclusions of the paper.
% Even though the content of the paper is presented in a very dense way, the assumptions of the models are adequately explained, the employed range of free parameters is clearly motivated and the outcome of the models is fairly compared to the observational results, using the right degree of caution to highlight the uncertainties associated with this comparison.
% Therefore I am in favor of recommending the present work for publication. Even if the first referee provided already different lengthy and detailed reports, I still have a few comments about the submitted work.

% - In Section 2.2 it is clearly stated that the stellar AM evolution models take into account also the torque exerted by the magnetospheric ejections (MEs), as parametrized in Gallet et al. (2019), whose peculiarity is that the sign of the torque depends on the relative position of the truncation radius with respect to the corotation radius. On the other hand the stellar angular momentum loss tends to be discussed by the authors in terms of the Accretion Powered Stellar Wind (APSW) efficiency only. For example I read at page 6, Section 3.2.2: “The APSW efficiency defines how much AM is removed from the star”. Or in the Discussion, Section 4.5: “Apart from APSW, other wind mechanisms can be important for the star and disk evolution”. But the MEs are exactly one of these mechanisms and are already included in the presented models. I understand that, since the MEs’ torque can change sign, going from spin-up to spin-down depending both on stellar and disk parameters, a discussion about their importance for the stellar angular momentum extraction can be tricky. Would it be possible to discuss their relevance more exhaustively? Is their effect in the presented AM evolution models negligible? Are they providing a spin-up effect only, thus leaving the APSW as the only spin-down mechanism? Is there a phase when they can extract stellar angular momentum? For example, when the mass accretion rate decreases, the truncation radius is expected to approach the corotation radius and gradually transit to a propeller regime, where the spin-down efficiency of the MEs is maximized. If there are any MEs spin-down phases, how their torque compares with the APSW? Could the MEs be one of the reasons why in the present work the authors can limit the stellar wind efficiency W to 5\%? The W = 10\% efficiency requirement is generally found in the literature assuming the APSW as the only stellar spin-down mechanism. I would like the authors to even just qualitatively discuss these aspects, either adding a subsection in the Discussion or inside Sections 3.1, 3.2.2 or 4.5.

> We agree that the effect of MEs is not discussed properly in the previous version and that the formulation of specific text phrases is misleading.
First, we added a more detailed description of the stellar spin model in Sec. 2.2.
To explain how different parameter configurations can affect the torque due to MEs, we added four paragraphs in Sec. 3.1. In addition, we compared the torque due to MEs based on our model for such configurations in Abstract A.1. Especially for fast-rotating stars and strong magnetic field strength toward the end of the disk lifetime, the MEs spin down the star. Compared to the torque due to the APSW, the torque due to MEs is comparable for fast-rotating stars and even the dominant source of stellar AM loss during the last >~1 Myr of the disk lifetime.

> The text phrases the referee found have been rewritten for clarity: In Sec. 3.2.2., we explicitly refer to the effects of different APSW efficiency values W. In Section 4.5., an additional sentence is added, mentioning the effects of MEs.






% - It is not compulsory, but I found confusing to find the observational arguments onto which the choice of the parameters of the models are based in the Discussion (Sections 4.1 and 4.2), therefore after that the choices for the stellar dipolar field strength and the initial mass accretion rates are presented at page 4. Analogously, Eq. (5) is shown way before the observational arguments onto which this formula is based and Fig. (8) are presented in the Discussion. Wouldn’t it be better to move the content of at least Section 4.1 and maybe also Section 4.2 to the place where the choice for the initial disk accretion rates and magnetic fields are shown at page 4?

> The arrangement of the sections defining the parameter space results from the revision history. We agree with the referee that it can be confusing. Thus, we follow the suggestion and put Sec. 4.1 and 4.2, as well as the old Eq. (5) that define the mass dependence of the initial accretion rate in Section 2.3.



% Two very minor points:

% - In the Conclusions section of the Abstract, I find the sentence “The scaling law between stellar SAM and the magnetic field strength is consistent for young stars, where all three parameters are constrained while motivating efforts to obtain more such measurements” a bit unclear. Which are the three parameters? Mass, SAM and magnetic field? Can this sentence be rephrased more clearly?

> The respective sentence in the abstract has been rephrased for clarity


% - The main text describing the solutions presented in Section 3.1 states that a W = 2\% parameter is employed, while the caption of Fig. 4 uses a W = 0 value, probably a typo from previous versions.

> This is indeed a typo and the value in the caption has been updated to 2\%









==> sections/eine_kleine_theorie.tex <==

The scaling relation we have derived from our model results (Eq. \ref{eq:combrel}) predicts that the specific angular momentum $j_\mathrm{final}$ of the star after the disk phase varies with the stellar mass and inversely with the strength of the stellar magnetic field. These overall trends can be intuitively understood as arising from: a stronger magnetic field driving greater loss of angular momentum from the star; and a more massive star having greater moment of inertia. If the disk is sufficiently massive such that the initial stellar spin is unimportant ("erasure" of initial conditions; \sref{sec:critical_mdot}) then a scaling relation could, in principle, be derived from the condition that further change in angular momentum of the star by the dissipating disk is negligible. This is the approach we adopt here.  


For a dissipating disk the accretion rate onto the star decreases. 
As a consequence, the inner disk radius, which is derived by balancing the stellar magnetic pressure with the ram pressure of the accreting disk material and gas pressure of the inner disk \citep[e.g.,][]{Romanova02,bessolaz08}, moves outwards. 
Stellar magnetic torques push the disk material just outside $r_\mathrm{cor}$ away from the star. 
The disk starts to pile up in this area since gas is still accreting from outer disk regions inwards \citep[][]{Steiner21}.
As the ram pressure decreases further (as $\Dot{M}_\mathrm{disk} \rightarrow 0$),  the relatively more important gas pressure in the inner disk can keep the inner disk radius close to the co-rotation radius and $r_\mathrm{in} \rightarrow r_\mathrm{cor}$ \citep[see Fig. 13 in][]{Steiner21}.
The stellar angular momentum evolution ($dJ/dt$) can then be approximated as
%
\begin{equation}\label{eq:dJdt}
     \frac{M_\star j}{\tau_\mathrm{j}} \propto \Gamma_\mathrm{ext} \, ,
\end{equation}
%
with the timescale $\tau_\mathrm{j}$ that is assumed to be to be of the order as the viscous disk lifetime.  
With $\Dot{M}_\mathrm{disk}\rightarrow 0$, $\Gamma_\mathrm{ext}$ includes only the magnetic star-disk connection and we can scale $j_\mathrm{final}$ by combining $\Gamma_\mathrm{ME} \propto B_\star^2 R_\star^6 r_\mathrm{in}^{-3}$ \citep[e.g.,][]{Armitage96,Gallet19} with \equ{eq:dJdt} 
%
\begin{equation}\label{eq:theo_j2}
    j_\mathrm{final} \propto B_\star^2 R_\star^6 M_\star^{-1} r_\mathrm{cor}^{-3} \tau_\mathrm{j} \, .
\end{equation}
%
The co-rotation radius $r_\mathrm{cor}$ scales with the specific angular momentum as
%
\begin{equation}\label{eq:theo_rcor}
    r_\mathrm{cor} \propto M_\star^{1/3} R_\star^{4/3} j^{-2/3}.
\end{equation}
%
Fits of power-law mass-radius relations to the isochrones of 0.15-0.6$M_{\odot}$ stars from the pre-main sequence model isochrones of \citet{Baraffe15} find $R_* \propto M_*^{\beta}$ where $\beta$ ranges from 0.22 at 1 Myr to 0.45 at 10 Myr.  Using this relation with \equ{eq:theo_j2}, \equ{eq:theo_rcor} becomes:
%
\begin{equation}
    j_\mathrm{final} \propto B_\star^{-2} M_\star^{2(1-\beta)} \tau_\mathrm{j}^{-1} \, .
\end{equation}
%
We arrive at the correct sense but exaggerated dependence of $j_\mathrm{final}$ on $B_\star$ and $M_\star$. While $\tau_\mathrm{j}$ usually scales with the viscous parameter $\alpha$, it is likely that $B_\star$ has an influence on this timescale.  A larger $B_\star$ will spin down the star, moving the co-rotation radius away from the star. Thus, more of the disk is located inside $r_\mathrm{cor}$ and is more rapidly accreted, decreasing $\tau_\mathrm{j}$ and attenuating the dependence on $B_\star$ (Gehrig~et~al. in prep).  All else being equal, a more massive star will spin down less rapidly due to its higher momentum of inertia; this keeps the co-rotation radius closer to the star, increasing $\tau_\mathrm{j}$ and decreasing the dependence of $j_\mathrm{final}$ on $M_\star$.  $\tau_\mathrm{j}$ also inversely depends on the disk viscous parameter $\alpha$ and thus we expect $j_\mathrm{final}$ to increase with increasing $\alpha$, as our model predicts (Figs. \ref{fig:j_Ball} and \ref{fig:j_M}).  
Finally, we point out that if stars begin their pre-main sequence lives with a mass-independent distribution of rotational periods, then the dependence of $j_\mathrm{final}$ on $M_\star$ in the case of no disk interaction can rise at least naturally since $j_\mathrm{final} \propto R_\star^2 \Omega_\star$ and $R_\star \propto M_\star^{1/3}$ (see above).

==> sections/newcommand_gen.tex <==
%\newcommand{\earth}{\mbox{$\oplus$}}

% Make Orcid icon
\definecolor{lime}{HTML}{A6CE39}
\DeclareRobustCommand{\orcidicon}{%
    \begin{tikzpicture}
    \draw[lime, fill=lime] (0,0) 
    circle [radius=0.16] 
    node[white] {{\fontfamily{qag}\selectfont \tiny ID}};
    \draw[white, fill=white] (-0.0625,0.095) 
    circle [radius=0.007];
    \end{tikzpicture}
    \hspace{-2mm}
}

\newcommand*{\tabhead}[1]{\multicolumn{1}{c}{\bfseries #1}}

\newcommand{\mystar}{{\Large {\fontfamily{lmr}\selectfont$\star$}}}

% Journals
\newcommand{\jgrp}{J. Geophys. Res.-Planets}
\newcommand{\rsos}{Royal Soc. Open Sci.}
\newcommand{\astrolett}{Astron. Lett.}

\newcommand{\usco}{Upper~Sco}
\newcommand{\rhooph}{$\rho$~Oph}
\newcommand{\oi}{[O\,I]}
\newcommand{\suii}{[S\,II]}
\newcommand{\nii}{[N\,II]}
\newcommand{\nai}{Na\,I}
\newcommand{\caii}{Ca\,II}
\newcommand{\mdotacc}{$\cdot{M}_{\rm acc}$}
\newcommand{\mdotwind}{$\cdot{M}_{\rm wind}$}
\newcommand{\hei}{He\,I}
\newcommand{\lyalpha}{Ly-$\alpha$}
\newcommand{\halpha}{H$\alpha$}
\newcommand{\mgi}{Mg\,I}
\newcommand{\sii}{Si\,I}

% Missions
\newcommand{\galex}{\emph{GALEX}}
\newcommand{\tess}{\emph{TESS}}
\newcommand{\plato}{\emph{PLATO}}
\newcommand{\gaia}{\emph{Gaia}}
\newcommand{\ktwo}{\emph{K2}}
\newcommand{\jwst}{\emph{JWST}}
\newcommand{\kepler}{\emph{Kepler}}
\newcommand{\corot}{\emph{CoRoT}}
\newcommand{\hipp}{\emph{Hipparcos}}
\newcommand{\spitzer}{\emph{Spizter}}
\newcommand{\herschel}{\emph{Herschel}}
\newcommand{\hst}{\emph{HST}}
\newcommand{\wise}{\emph{WISE}}


% astronomical objects
\newcommand{\twa}{TW Hydra}
\newcommand{\bpic}{$\beta$~Pictoris}
\newcommand{\abdor}{AB~Doradus}
\newcommand{\rup}{Ruprecht~147}
\newcommand{\etacha}{$\eta$\,Chamaeleontis}


\newcommand{\doar}{DoAr\,25}
\newcommand{\epcha}{EP\,Cha}
\newcommand{\rylup}{RY\,Lup}
\newcommand{\hdtwofour}{HD\,240779}

% parameters
\newcommand{\sigrv}{$\sigma_{\rm RV}$}

% units
\newcommand{\etal}{\mbox{\rm et al.~}}
\newcommand{\ms}{\mbox{m\,s$^{-1}~$}}
\newcommand{\kms}{\mbox{km\,s$^{-1}~$}}
\newcommand{\ks}{\mbox{km\,s$^{-1}~$}}
\newcommand{\kse}{\mbox{km\,s$^{-1}$}}
\newcommand{\mse}{\mbox{m\,s$^{-1}$}}
\newcommand{\msy}{\mbox{m\,s$^{-1}$\,yr$^{-1}~$}}
\newcommand{\msye}{\mbox{m\,s$^{-1}$\,yr$^{-1}$}}
\newcommand{\msun}{M$_{\odot}$}
\newcommand{\msune}{M$_{\odot}$}
\newcommand{\rsun}{R$_{\odot}$}
\newcommand{\lsun}{L$_{\odot}~$}
\newcommand{\rsune}{R$_{\odot}$}
\newcommand{\mjup}{M$_{\rm JUP}~$}
\newcommand{\mjupe}{M$_{\rm JUP}$}
\newcommand{\msat}{M$_{\rm SAT}~$}
\newcommand{\msate}{M$_{\rm SAT}$}
\newcommand{\mnep}{M$_{\rm NEP}~$}
\newcommand{\mnepe}{M$_{\rm NEP}$}
%\newcommand{\mearth}{M$_{\rm Earth}~$}
%\newcommand{\mearthe}{M$_{\rm Earth}$}
\newcommand{\mearth}{$M_{\oplus}$}
\newcommand{\mearthe}{$M_{\oplus}$}
\newcommand{\rearth}{$R_{\oplus}$}
\newcommand{\rearthe}{$R_{\oplus}$}
\newcommand{\rjup}{R$_{\rm JUP}~$}
%\newcommand{\msini}{$M \sin i~$}
\newcommand{\msinie}{$M_{\rm p} \sin i$}
%\newcommand{\vsini}{$V \sin i~$}
\newcommand{\vsinie}{$V \sin i$}
\newcommand{\mbsini}{$M_b \sin i~$}
\newcommand{\mcsini}{$M_c \sin i~$}
\newcommand{\mdsini}{$M_d \sin i~$}
\newcommand{\chisq}{$\chi_{\nu}^2$}
\newcommand{\chinu}{$\chi_{\nu}$}
\newcommand{\chinusq}{$\chi_{\nu}^2$}
\newcommand{\arel}{$a_{\rm rel}$}
%\newcommand{\teff}{${\rm T_{eff}}$}
\newcommand{\feh}{\ensuremath{[\mbox{Fe}/\mbox{H}]}}
\newcommand{\rphk}{\ensuremath{R'_{\mbox{\scriptsize HK}}}}
\newcommand{\lrphk}{\ensuremath{\log{\rphk}}}
%\newcommand{\caii}{\ion{Ca}{2} H \& K}
%\newcommand{\caiih}{\ion{Ca}{2} H}
\newcommand{\mv}{\ensuremath{M_{\mbox{\scriptsize V}}}}
\newcommand{\cs}{$\sqrt{\chi^2_{\nu}}$}
\newcommand{\etaearth}{$\mathbf \eta_{\oplus} ~$}
\newcommand{\etaearthe}{$\mathbf \eta_{\oplus}$}

\newcommand{\sini}{\ensuremath{\sin i}}
\newcommand{\msini}{\ensuremath{M_{\rm p} \sin i}}
\newcommand{\mplsini}{\ensuremath{\mpl\sin i}}
\newcommand{\teff}{\ensuremath{T_{\rm eff}}}
\newcommand{\teq}{\ensuremath{T_{\rm eq}}}
\newcommand{\logg}{\ensuremath{\log{g}}}
\newcommand{\vsini}{\ensuremath{v \sin{i}}}
\newcommand{\ebv}{E($B$-$V$)}

% -------- Aliases specific to Kepler or Kepler diagnostics -------------
\newcommand{\Kepler}{\emph{Kepler}~}
\newcommand{\Keplere}{\emph{Kepler}}
\newcommand{\blender}{{\tt BLENDER}~}


% -------- Aliases about the star properties  -------------
%\newcommand{\kp}{\ensuremath{K_{p}}}
\newcommand{\kp}{\ensuremath{\mathrm{Kp}}}
\newcommand{\rstar}{\ensuremath{R_\star}}
\newcommand{\mstar}{\ensuremath{M_\star}}
\newcommand{\loggstar}{\ensuremath{\logg_\star}}
\newcommand{\lstar}{\ensuremath{L_\star}}
\newcommand{\astar}{\ensuremath{a_\star}}
\newcommand{\loglstar}{\ensuremath{\log{L_\star}}}
\newcommand{\rhostar}{\ensuremath{\rho_\star}}

% -------- Aliases about planet properties -------------
\newcommand{\rp}{\ensuremath{R_{\rm p}}}
\newcommand{\rpl}{\ensuremath{r_{\rm P}}~}
\newcommand{\rple}{\ensuremath{r_{\rm P}}}
\newcommand{\mpl}{\ensuremath{m_{\rm P}}~}
\newcommand{\lpl}{\ensuremath{L_{\rm P}}~}
\newcommand{\rhopl}{\ensuremath{\rho_{\rm P}}~}
\newcommand{\loggpl}{\ensuremath{\logg_{\rm P}}~}
\newcommand{\logrpl}{\ensuremath{\log r_{\rm P}}~}
\newcommand{\logrple}{\ensuremath{\log r_{\rm P}}}
\newcommand{\loga}{\ensuremath{\log a}~}
\newcommand{\logmpl}{\ensuremath{\log m_{\rm P}}~}



